Improving End-to-end Speech Recognition with Pronunciation-assisted Sub-word Modeling

Most end-to-end speech recognition systems model text directly as a sequence of characters or sub-words. Current approaches to sub-word extraction only consider character sequence frequencies, which at times produce inferior sub-word segmentation that might lead to erroneous speech recognition output. We propose pronunciation-assisted sub-word modeling (PASM), a sub-word extraction method that leverages the pronunciation information of a word. Experiments show that the proposed method can greatly improve upon the character-based baseline, and also outperform commonly used byte-pair encoding methods.

==> Improving End-to-end Speech Recognition with Pronunciation-assisted Sub-word Modeling/Makefile <==

all: paper.pdf	
#	cp paper.pdf interspeech2015_multitree.pdf
	open paper.pdf

paper.pdf: IEEEbib.bst spconf.sty paper.tex refs.bib *.png
	pdflatex paper
	bibtex paper || true
	pdflatex paper
	pdflatex paper

clean:
	@rm -f paper.aux paper.bbl paper.blg paper.dvi \
	paper.log paper.pdf paper.ps paper.pdf


==> Makefile <==

all: paper.pdf	
#	cp paper.pdf interspeech2015_multitree.pdf
	open paper.pdf

paper.pdf: IEEEbib.bst spconf.sty paper.tex refs.bib *.png
	pdflatex paper
	bibtex paper || true
	pdflatex paper
	pdflatex paper

clean:
	@rm -f paper.aux paper.bbl paper.blg paper.dvi \
	paper.log paper.pdf paper.ps paper.pdf

